Bootstrapping Reinforcement Learning with Imitation for Vision-Based Agile Flight

Learning visuomotor policies for agile quadrotor flight presents significant difficulties, primarily from inefficient policy exploration caused by high-dimensional visual inputs and the need for precise and low-latency control. To address these challenges, we propose a novel approach that combines the performance of Reinforcement Learning (RL) and the sample efficiency of Imitation Learning (IL) in the task of vision-based autonomous drone racing. While RL provides a framework for learning high-performance controllers through trial and error, it faces challenges with sample efficiency and computational demands due to the high dimensionality of visual inputs. Conversely, IL efficiently learns from visual expert demonstrations, but it remains limited by the expert's performance and state distribution. To overcome these limitations, our policy learning framework integrates the strengths of both approaches. Our framework contains three phases: training a teacher policy using RL with privileged state information, distilling it into a student policy via IL, and adaptive fine-tuning via RL. Testing in both simulated and real-world scenarios shows our approach can not only learn in scenarios where RL from scratch fails but also outperforms existing IL methods in both robustness and performance, successfully navigating a quadrotor through a race course using only visual information. Videos of the experiments are available at https://rpg.ifi.uzh.ch/bootstrap-rl-with-il/index.html.

==> figures/tex/critic_prev.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/tex/critic_prev.pdf}
%    \vspace*{-4pt}
    \caption{\rss{Reward visualization for the SplitS track using policies from pixels with ResNet w/ and w/o pre-trained critic function.}}
    \label{fig:critic_prev}
    \vspace{-0.5cm}
\end{wrapfigure}

==> figures/tex/dagger_loss.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}    
    \centering
    \includegraphics[width=\linewidth]{figures/supplementary/dagger_loss.pdf}
%    \vspace*{-4pt}
    \caption{\corl{Illustration of the training loss of the IL policy on \emph{SplitS Track} with DAgger.}}
    \label{fig:dagger}
    \vspace{-3pt}
\end{wrapfigure}

==> figures/tex/drone.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/supplementary/drone.png}
    \caption{Our hardware drone platform for HIL experiments in the real world.}
    \label{fig:drone}
\end{figure}

==> figures/tex/eyecatcher.tex <==
\makeatletter
\g@addto@macro\@maketitle{
  \captionsetup{type=figure}\setcounter{figure}{0}
  \def\mycolspace{1.2mm}
  \centering
  \tikzset{font=\small}
  \begin{tikzpicture}
    % \newcommand\xa{0.25}
    \newcommand\xb{0}
    \newcommand\xa{-4.5}

    \node [inner sep=0pt, outer sep=0pt] (img1) at (-2+\xb,0) 
    {\includegraphics[width=0.74\linewidth]{figures/pictures/eyecatcher/overlay.png}};
    
    \node [inner sep=0pt, outer sep=2pt] (img2) at (9.3 + \xa, 0.3)
    {\includegraphics[width=0.2\linewidth]{figures/pictures/eyecatcher/violinplot.pdf}};
    \node [rotate=45] at (9.1+ \xa, -3) {\textcolor{RedOrange}{DAgger}};
    \node [rotate=45] at (9.6+ \xa, -2.5) {~\cite{ross2011dagger}};
    \node [rotate=45, align=center] at (8.0+ \xa, -2.9) {Behavior\\ Cloning};
    \node [rotate=45] at (10.4+ \xa, -2.8) {\textbf{\textcolor{RoyalBlue}{Ours}}};
    \node [rotate=90] at (6.9+ \xa, 0.4) {Lap Time [s]};
    \node[draw=blue!30, fill=blue!5, rounded corners, rectangle, align=center, line width=0.4pt] at (9.2+ \xa, -1.6) {$\mu$:8.06};
    \node[draw=blue!30, fill=blue!5, rounded corners, rectangle, align=center, line width=0.4pt] at (10.35+ \xa, -1.6) {$\mu$:7.67};

    \node[draw=gray!70, fill=gray!10, rounded corners, rectangle, align=center, line width=0.4pt,  rotate=90] at (8.2+ \xa, 0.3) { \qquad\quad \quad Not able to fly\qquad\qquad\;    };

    \node at (7.35+ \xa, -1.7) {7.4};
    \node at (7.35+ \xa, -0.58) {7.6};
    \node at (7.35+ \xa, 0.46) {7.8};
    \node at (7.35+ \xa, 1.52) {8.0};
    \node at (7.35+ \xa, 2.58) {8.2};
    \node at (7.35+ \xa, 2.58) {8.2};
    % legend
    % \node[draw=blue!30, fill=blue!2,  rectangle, align=left, line width=0.4pt] at (-5.93+\xb, -2.9) {\textcolor{RoyalBlue}{Ours}\\ \textcolor{WildStrawberry}{DAgger}~\cite{ross2011dagger}};
    \node[draw=blue!30, fill=blue!2,  rectangle, align=left, line width=0.4pt] at (-5.9+\xb, 2.7) {\textcolor{RoyalBlue}{Ours}\\ \textcolor{RedOrange}{DAgger}~\cite{ross2011dagger}};
\end{tikzpicture}
    \vspace{1.0ex}
	\captionof{figure}{\textit{Left:} Trajectory visualization of the Imitation Learning (IL) (red) and our Reinforcement Learning (RL) fine-tuned (blue) vision-based policies from our real-world, drone-racing experiments. Both policies utilize only visual observations as network inputs and can complete the race track. Trained with the same amount of data, our RL fine-tuned policy demonstrates the ability to execute tighter trajectories and fly faster. \textit{Right:} Our policy consistently demonstrates faster flight in real-world scenarios over 10 consecutive laps, with a lap-time advantage of approximately 0.4 seconds over imitation learning alone. This margin can prove decisive in drone-racing championships where a tenth of a second can make the difference.}
%  \davide{While I find the picture artistic, it doesn't convey our contribution. I only see a doodle. Why don't you replace it with a picture of a drone flying through some gates, with a single-lap trajectory obtained from imitation learning in blue and the corresponding one from our approach in red? Blue and green are too similar. The background should be well-lit; it is impossible to understand what is going on.}
% \davide{The plot on the right is confusing: move the label of the y-axis to the left side of the vertical axis (left of the numbers). Change BC to Behavior Cloning. Point out in the caption that in drone racing the difference between first and second place winner is a tenth of a second, so the improvement in lap time is significant.. }
% \davide{Please rewrite the caption as follows: (1) what we do in this paper and (2) what the picture shows.}
\vspace{-2pt}
\label{fig:catcheye}
}
\makeatother

==> figures/tex/forget.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/tex/forget.pdf}
%    \vspace*{-4pt}
    \caption{\rss{Reward visualization for the SplitS track using policies from pixels with ResNet. We could observe that by using the vanilla bootstrapping strategy, the policy learning process will lead to catastrophic forgetting. Hence we highlight the importance of the adaptivity of our approach.}}
    \label{fig:forget}
    \vspace{-3pt}
\end{wrapfigure}

==> figures/tex/imtation.tex <==
\begin{figure*}[bt]
    \centering
\includegraphics[width=\linewidth]{figures/pictures/imitation.pdf}
\vspace{2pt}\caption{\corl{\emph{Top:} Trajectory and action errors visualization for the two different IL approaches applied to vision-based drone racing. \emph{Bottom:} Normalized control command output visualization, from bottom to end: Collective thrust, $\omega_x$, $\omega_y$, $\omega_z$, normalized in the range of $[-1, 1]$. In (a), even trained with more data samples, the policy cannot manage to consistently pass the first gate. Conversely, using DAgger, we can clearly observe that the policy could eventually fly through the gates, and using more data, the policy gets consistent improvement. All these policies are then used for the RL fine-tuning as illustrated in Fig.~\ref{fig:init_reward}}.}
\label{fig:imitation}
\end{figure*}

==> figures/tex/lr.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\linewidth]{figures/supplementary/lr/lr.pdf}
    \includegraphics[width=0.49\linewidth]{figures/supplementary/dagger_loss.pdf}
    \caption{\corl{\textbf{Left:}Learning rate visualization of our adaptive RL fine-tuning stage. \textbf{Right:}Illustration of the training loss of the IL policy on \emph{SplitS Track} with DAgger.}}

    % \vspace{-1cm}
    \label{fig:lr}
\end{figure}

==> figures/tex/percentage_ablation.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    % \vspace{-0.6cm}
    \includegraphics[width=\linewidth]{figures/pictures/corner_racing/percentage_ablation.pdf}
    \caption{Rewards visualization for the SplitS track using policies from pixels with ResNet. By varying percentages (from 10\% to 90\%) of DAgger policies in fine-tuning using our proposed approach. Our approach reveals substantial benefits, even with 15\% of data samples for policy training.}
    \label{fig:init_reward}
    \vspace{-10pt}
\end{wrapfigure}

==> figures/tex/percentage_rollout.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/pictures/corner_racing/reward.pdf}
%    \vspace*{-4pt}
    \caption{Using a fixed sample budget, we varied the IL policy percentage for our approach on the vision-based policy for SplitS track, achieving a local maximum in deployment reward with 60$\%$ IL pretraining and 40$\%$ RL fine-tuning.}
    \label{fig:percentage_rollout}
    \vspace{-0.2cm}
\end{wrapfigure}

==> figures/tex/rss_track.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/pictures/race_tracks/rss.png}
    \caption{Illustration of the longer range \textit{RSS} track.}
    \label{fig:rss_track}
\end{figure}

==> figures/tex/state_rl.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    % \vspace{-0.5cm}
    \includegraphics[width=\linewidth]{figures/supplementary/ours_vs_states.pdf}
    \caption{Comparing rewards of the visuomotor policy using our approach and the state-based policy. }
    \label{fig:state}
    % \vspace{0.5cm}
\end{wrapfigure}

==> tables/states.tex <==
\begin{table*}[!htp]
    \centering
    \small
    \caption{\corl{Policy performance evaluation averaged by 6 different history lengths using both implicitly learned representations, specifically a common ResNet50~\cite{he2016deep} for RGB images, and the task-specific gate corners positions across three different racing tracks. We demonstrate that the average performance of our approach surpasses all baselines.}}
    \label{tab:states}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{ccc|cc|cc}
    \toprule
      \multirow{3}*{\textbf{Methods}} & \multicolumn{6}{c}{\textbf{Race Tracks}}\\
    &\multicolumn{2}{c|}{\textit{Figure 8}}& \multicolumn{2}{c|}{\textit{SplitS}} & \multicolumn{2}{c}{\textit{Kidney}}\\
    & MGE [m] & LT [s]& MGE [m] & LT [s]& MGE [m] & LT [s]\\
    \midrule
   State-based  & 0.13& 4.52  & 0.09 & 7.75  & 0.12 & 4.90\\ 
                         
    Ours   & 0.32 & 4.57 & 0.25 & 7.77 & 0.21 &  4.93\\
    \bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table*}
